Lessons learned in multilingual grounded language learning

Recent work has shown how to learn better visual-semantic embeddings by leveraging image descriptions in more than one language. Here, we investigate in detail which conditions affect the performance of this type of grounded language learning model. We show that multilingual training improves over bilingual training, and that low-resource languages benefit from training with higher-resource languages. We demonstrate that a multilingual model can be trained equally well on either translations or comparable sentence pairs, and that annotating the same set of images in multiple language enables further improvements via an additional caption-caption ranking objective.

==> charts.tex <==
\begin{figure*}
\begin{center}
\begin{tikzpicture}%[yscale=0.55, xscale=0.55]

\begin{groupplot}[
   group style={
       group size=2 by 1,
       x descriptions at=edge bottom,
       y descriptions at=edge left,
       vertical sep=0pt,
       horizontal sep=15pt},
  ybar,
  x=2.3cm,
  every node near coord/.append style={font=\normalsize},
  nodes near coords,
  nodes near coords align=vertical,
  enlarge x limits=0.2,
  %xmajorgrids = true,
  point meta=y * 1, % The displayed number.
  ylabel={\textbf{R@10}},
  tick align=outside,
  ytick={0,20,...,100}, 
  xtick={1,...,3},
  xticklabels={
    Monolingual,
    Bilingual,
    Multilingual},
  x tick label style={align=left},
  ymin=0,
  ymax=100
]

\nextgroupplot[bar width=18pt]
\addplot[draw=red,fill=red!50]
coordinates {(1,56.3) (2,67.6) (3,71.9)};
\addplot[draw=blue, fill=blue!50] 
coordinates {(1,40.1) (2,56.0) (3,61.0)};
\node at (rel axis cs:0.5,0.9) {English};

\nextgroupplot[bar width=18pt,legend style={at={(-0.05,1)},anchor=north}]
\addplot[draw=red,fill=red!50]
coordinates {(1,39.5) (2,61.9) (3,65.1)};
\addlegendentry{I $\rightarrow$ T}
\addplot[draw=blue, fill=blue!50] 
coordinates {(1,20.9) (2,49.1) (3,52.6)};
\addlegendentry{T $\rightarrow$ I}

\node at (rel axis cs:0.5,0.9) {German};
\end{groupplot}
\end{tikzpicture}
\caption{Comparing best models from the Bilingual and Multilingual settings on the
T2 test set. The Bilingual and Monolingual models are trained on the 
downsampled T2 English and German sets with additional c2c objective as this setup
provided the overall best results. The Multilingual model takes the T1 French and
Czech as additional training data.}
\end{center}
\end{figure*}

